Electromagnetic Modelling of Extended Targets in a Distributed Antenna System

Traditional radar and integrated sensing and communication (ISAC) systems often approximate targets as point sources, a simplification that fails to capture the essential scattering characteristics for many applications. This paper presents a novel electromagnetic (EM)-based framework to accurately model the near-field (NF) scattering response of extended targets, which is then applied to three canonical shapes : a flat rectangular plate, a sphere and a cylinder. Mathematical expressions for the received signal are provided in each case. Based on this model, the influence of bandwidth, carrier frequency and target distance on localisation accuracy is analysed, showing how higher bandwidths and carrier frequencies improve resolution. Additionally, the impact of target curvature on localisation performance is studied. Results indicate that detection performance is slightly enhanced when considering curved objects. A comparative analysis between the extended and point target models shows significant similarities when targets are small and curved. However, as the target size increases or becomes flatter, the point target model introduces estimation errors owing to model mismatch. The impact of this model mismatch as a function of system parameters is analysed, and the operational zones where the point abstraction remains valid and where it breaks down are identified. These findings provide theoretical support for experimental results based on point-target models in previous studies.

==> ml_estimation.tex <==

This section builds on the general EM signal model developed in Section~\ref{sec:system_model} to present a new estimator for the 3D localisation of the target, i.e. an estimation of the range $R$, azimuth angle $\phi$, and elevation angle $\theta$ between the centre of the antenna array and the target. 

\subsection{Range and Angles Estimation}






Similarly to \cite{moulin_near-field_2024}, with an orthogonal transmission, the received signal $u_{l'l}$ transmitted at the $l$-th antenna and received at the $l'$-th antenna is written as  
\begin{equation}
    u_{l'l}(t) = \xi \: \mu_{l^{\prime} l ; R, \phi, \theta}(t)+w_{l^{\prime}l}(t),
\end{equation}
where $w_{l'l}(t)$ is an Additive White Gaussian Noise (AWGN), $\xi$ is a random complex coefficient identical for all antennas and  $\mu_{l^{\prime} l; R, \phi, \theta}(t)$ is the model of the signal at the $l'$-th receiving antenna from the $l$-th transmitting antenna, defined here as 
\begin{align}
    &\mu_{l^{\prime} l ; R, \phi}(t)= 
    \sum_{\substack{\mathbf{x}_0 \\ \nabla \psi(\mathbf{x}_0) = 0}}^{} 
    g(\mathbf{x}_0) \, e^{j k \psi(\mathbf{x}_0)} 
    \left( \frac{2 \pi}{k} \right)^{n/2} \\
\nonumber     &\quad \cdot \left| \det \nabla^2 \psi(\mathbf{x}_0) \right|^{-1/2} 
      e^{j \frac{\pi}{4} \, \operatorname{sgn}(\nabla^2 \psi(\mathbf{x}_0))} s_{l}\left(t- \frac{r_{ls} + r_{l's}}{c}\right). 
\end{align}
The positions of the stationary points \( \mathbf{x}_0 \) are derived in Section~\ref{sec:SPA}, and depend on the positions of the antenna pair \( l \) and \( l' \) and can be expressed as functions of $R$, $\phi$ and $\theta$. 


Based on the developments of \cite{moulin_near-field_2024} for the rectangular plate and parallel linear array, the 3D localisation problem can be rewritten following the ML approach as
\begin{equation}
    \hat{R}, \hat{\phi}, \hat{\theta} = \arg \max_{R, \phi, \theta} \frac{\left|\sum_{l^{\prime}=0}^{N-1} \sum_{l=0}^{N-1} \int_t u_{l^{\prime} l}(t) \mu_{l^{\prime} l ; R}^*(t) \mathrm{d} t\right|^2}{\sum_{l^{\prime}=0}^{N-1} \sum_{l=0}^{N-1} \int_t\left|\mu_{l^{\prime} l ; R}(t)\right|^2 \mathrm{~d} t}.  
\end{equation}

It should be noted that, unlike the range estimator presented in \cite{moulin_near-field_2024}, this study considers an arbitrary shape for the target and arbitrary positions of the antennas. 
Moreover, in addition to the range, the angles $\phi$ and $\theta$ are also estimated in this new problem, enabling the localisation of the target. 

Note also that similar reasoning can be applied to the non-orthogonal case, i.e. when the signals $s_l$ are not orthogonal.


\subsection{Numerical Results}



\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth, trim=0 0 50 0, clip]{ML_R_phi_20_bis_bis_without_edges.pdf}
    \caption{2D Ambiguity function of the ML estimator for $\tilde{\theta} = \theta$ for a spherical target. }
    \label{fig:ambiguity_function}
\end{figure}

Figure \ref{fig:ambiguity_function} illustrates the ambiguity function for estimating the range $R$ and the azimuth angle $\phi$ when $\tilde{\theta} = \theta$ in the case of a spherical target, when the elevation and azimuth angles are both equal to zero. %
Compared to the parameters described in Table~\ref{tab:parameters}, here the number of antennas is set to $20$, and they are still aligned along the $z$-axis.

The ML function shows a maximum for both the range and angle estimations located at their true values, indicating that the estimator is able to accurately localise the target. The peaky nature of the maximum can be explained by the maximum likelihood formulation of the estimator. However, for the angle estimation, several secondary peaks can be observed. These are grating lobes due to the small number of antennas and the large antenna spacing considered in this scenario, and they can be for instance reduced by increasing the number of antennas. Note that similar results are obtained considering the estimation of the elevation angle $\theta$ for $\tilde{\phi} = \phi$.

